The Anatomy of Electro-Weak Symmetry Breaking. I: The Higgs boson in the Standard Model

This review is devoted to the study of the mechanism of electroweak symmetry breaking and this first part focuses on the Higgs particle of the Standard Model. The fundamental properties of the Higgs boson are reviewed and its decay modes and production mechanisms at hadron colliders and at future lepton colliders are described in detail.

==> sm4/hsm4-refs.tex <==
%%%%%%%%%%%%%%%%%%%%%% Section 4.1: Introduction %%%%%%%%%%% 



\bibitem{TESLAtdr} J. Andruszkow et al, TESLA Technical Design Report, Part II,
{\it The Accelerator}, DESY 2001-011, ECFA 2001-209

\bibitem{NLCtdr} {\it Zeroth Order Design Report for the Next Linear Collider},
SLAC Report 474, 1996; {\it 2001 Report on the Next Linear Collider},
Fermilab-Conf-01-075-E. 

\bibitem{JLCtdr} KEK-Report 97-1, 1997.

\bibitem{CLICtdr} R.W.~Assmann et al.,``{\it A 3-TeV $\ee$  linear collider 
based on CLIC technology}", CERN-2000-008.

\bibitem{eeReviews} Selected reviews for machine and detector physics. 

\bibitem{TESLA} J.A. Aguilar-Saavedra et al, TESLA Technical Design Report, 
Part III, {\it Physics at an $e^+e^-$ Linear Collider}, hep-ph/0106315.

\bibitem{NLC} T. Abe et al, {\it Linear Collider Physics Resource Book for 
Snowmass 2001}, hep-ex/0106055-58.

\bibitem{JLC} K. Abe et al, {\it Particle Physics Experiments at JLC},
hep-ph/0109166.

\bibitem{CLIC} CLIC Report. 

\bibitem{gamma-machine} I.~Ginzburg, G.~Kotkin, V.~Serbo and V.~Telnov, 
Pizma ZhETF 34 (1981) 514 and JETP Lett. 34 (1982) 491;
I.~Ginzburg, G.~Kotkin, V.~Serbo and V.~Telnov, Nucl.  Instr. \& Meth. 
205 (1983) 47.

\bibitem{gamma-machine2} I.~Ginzburg, G.~Kotkin, S.~Panfil, V.~Serbo and 
V.~Telnov, Nucl. Instr. Meth. 219 (1984) 5.
%
\bibitem{gammaReview} Review on gamma-machines. 
%
\bibitem{muonReview} Review on muons colliders. 

%%%%%%%%%%%%%%%%%%%%%%%%%Section 4.2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{EGN} 
J. Ellis, M.K. Gaillard, and D.V. Nanopoulos, Nucl. Phys.  B106 (1976) 292.
%
\bibitem{LQT}
B.W. Lee, C. Quigg and H.B. Thacker, Phys. Rev. D16 (1977) 1519.
%
\bibitem{Bjorken-process} 
J.D. Bjorken, Proc. 1976 SLAC Summer Inst. Part. 
Phys., ed. M.C. Zipf (SLAC report 198,1977) 1. 
%
\bibitem{Higgs-strahlung}
B.L. Joffe and V.A. Khoze, Sov. J. Part. Phys. {\bf 9} (1978) 50; 
D.R.T. Jones and S.T. Petcov, Phys. Lett. B84 (1979) 440; 
F.A. Behrends and R. Kleiss, Nucl. Phys. B260 (1985) 32.
%
\bibitem{Wfus1}
R.N.\ Cahn and S.\ Dawson, Phys.\ Lett.\ B136 (1984) 196; 
K.\ Hikasa, Phys.\ Lett.\ B164 (1985) 341. 

\bibitem{Wfus2}
G.\ Altarelli, B.\ Mele and F.\ Pitolli, Nucl.\ Phys.\ B287 (1987) 205.

\bibitem{Wfus3} W. Kilian, M. Kr\"amer and P.M. Zerwas, Phys. Lett. B373 
(1996) 135.
%
\bibitem{ttH1} Old ttH
%
\bibitem{ttH2} Our ttH. 
%
\bibitem{HHZ1} Old HHZ, Haber et al. 
% 
\bibitem{HHW1} Old HHW
%
\bibitem{DKMZ} Maggies paper.
%
\bibitem{Hgamma1} Old Hgamma.
%
\bibitem{Hgamma2} Our Hgamma.
%
\bibitem{HHloop1} Old HH from loop.
%
\bibitem{HHloop2} Our HH from loop. 
%
\bibitem{HVVprod} HVV production.
%
\bibitem{Hffprod} Hff production.
%
\bibitem{HppP1}
%
\bibitem{HppP2}
%
\bibitem{HppP3}
%
\bibitem{egammaP}
%
\bibitem{mumuP1}
%
\bibitem{mumuP2}
%
\bibitem{RCHZ} 
J. Fleischer and F. Jegerlehner, Nucl. Phys. B216 (1983) 469;
B. A. Kniehl, Z. Phys. C55 (92) 605;
A. Denner, J. K\"ublbeck, R. Mertig and M. B\"ohm, Z. Phys. C56 (92) 261.
%
\bibitem{RCWW1} 
A. Denner, S. Dittmaier, M. Roth and M. M. Weber, Nucl. Phys. B660 (2003) 289.

\bibitem{RCWW2} 
G. B\'elanger, F. Boudjema, J. Fujimoto, T. Ishikawa, T. Kaneko, 
K. Kato and Y. Shimizu, Phys. Lett. B559 (2003) 252. 

\bibitem{RCWW3} F. Jegerlehner and O. Tarasov, Nucl. Phys. Proc. Suppl. 116 
(2003) 83.  

\bibitem{RCZZ} F. Boudjema, J. Fujimoto, T. Ishikawa, T. Kaneko, K. Kato
Y. Kurihara, Y. Shimizu, S. Yamashita, Y. Yasui, hep-ph/0404098. 

\bibitem{RCTTqcd1} S. Dittmaier, M. Kr\"amer, Y. Liao, M. Spira and P.M. Zerwas,
Phys. Lett. B441 (1998) 383. 

\bibitem{RCTTqcd2} S. Zhu, hep-ph/0212273;  for the correction to the dominant
channel see also S. Dawson and L. Reina,  Phys. Rev. D59 (1999) 054012.

\bibitem{RCTTew1} G. B\'elanger, F. Boudjema, J. Fujimoto, T. Ishikawa, 
T. Kaneko, K. Kato, Y. Shimizu and Y. Yasui, Phys. Lett. B571 (2003) 163; 

\bibitem{RCTTew2}
A. Denner, S. Dittmaier, M. Roth and  M.M. Weber, Phys. Lett. B575 (2003) 290.

\bibitem{RCTTew0}
You Yu, Ma Wen-Gan, Chen Hui, Zhang Ren-You, Sun Yan-Bin and Hou Hong-Sheng,
Phys. Lett. B571 (2003) 85.

\bibitem{RCZHH}  G. B\'elanger, F. Boudjema, J. Fujimoto, T. Ishikawa, 
T. Kaneko, Y. Kurihara, K. Kato and Y. Shimizu, Phys. Lett. B576 (2003) 152;
Zhang Ren-You, Ma Wen-Gan, Chen Hui, Sun Yan-Bin and Hou Hong-Sheng,
Phys. Lett. B578 (2004) 349.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{High-Precision} The LEP Collaborations (ALEPH, DELPHI, L3 and OPAL), 
the LEP Electroweak Working Group and the SLD Heavy Flavour Group, {\it A
combination of preliminary Electroweak measurements and constraints on the
Standard Model}, hep-ex/0312O23; {\tt http://lepewwg.web.cern.ch/LEPEWWG};
for an update see, G. Altarelli and M. Grunewald, hep-ph/0404165.
% 
\bibitem{MW-Tevatron} The CDF and D0 collaborations, hep-ex/0311039.
%
\bibitem{Mt-Tevatron} The CDF and D0 collaborations and the Tevatron 
Electroweak Working Group, hep-ex/0404010.
%
\bibitem{alphas-review} G. Altarelli, hep-ph/0204179;
S. Bethke, Nucl. Phys. Proc.Suppl. 121 (2003) 74 [hep-ex/0211012];
I. Hinchliffe in Ref.~\cite{PDG}.
%
\bibitem{PDG} Particle Data Group, K. Hagiwara et al., Phys. Rev. D66 
(2002) 010001.
%
\bibitem{Z-Physics} {\it Z Physics at LEP1}, CERN Report 89--08 (1989),
eds. G. Altarelli, R. Kleiss and C. Verzegnassi; see this reference for 
earlier work. 
%
\bibitem{W-Physics} {\it Physics at LEP2}, CERN Report 96--01, eds. G. 
Altarelli, T. Sj\"ostrand and F. Zwirner.  
%
\bibitem{Bjorken-process} 
J.D. Bjorken, Proc. 1976 SLAC Summer Inst. Part. 
Phys., ed. M.C. Zipf (SLAC report 198,1977) 1. 
%
\bibitem{Z-h-gamma1} R.N. Cahn, M.S. Chanowitz and N. Fleishon, Phys. Lett.
82B (1979) 113. 
%
\bibitem{Z-h-gamma2} L. Bergstrom and G. Hulth, Nucl. Phys. B259 (1985) 137.
% 
\bibitem{EGN} 
J. Ellis, M.K. Gaillard, and D.V. Nanopoulos, Nucl. Phys.  B106 (1976) 292.
%
\bibitem{LQT}
B.W. Lee, C. Quigg and H.B. Thacker, Phys. Rev. D16 (1977) 1519.
%
\bibitem{Higgs-strahlung}
B.L. Joffe and V.A. Khoze, Sov. J. Part. Phys. {\bf 9} (1978) 50; 
D.R.T. Jones and S.T. Petcov, Phys. Lett. B84 (1979) 440; 
F.A. Behrends and R. Kleiss, Nucl. Phys. B260 (1985) 32.
%
\bibitem{LEP2-Higgs-Th} M. Carena, Peter M. Zerwas (conv.) et al., 
{\it Higgs Physics at LEP2} in \cite{W-Physics}, 
Part I, p. 351 [hep-ph/9602250]. 
%
\bibitem{LEP2-Higgs-exp} The LEP Collaboration (ALEPH, DELPHI, L3 and OPAL), 
Phys. Lett. B565 (2003) 61 [hep-ex/0306033]. 
%
\bibitem{LEP2-Higgs-ind} The LEP Collaboration (ALEPH, DELPHI, L3 and OPAL), 
hep-ex/0107032 (invisible decays) and hep-ex/0107034 (flavor blind hadronic 
decays). 


